The Power of Summary-Source Alignments

Multi-document summarization (MDS) is a challenging task, often decomposed to subtasks of salience and redundancy detection, followed by text generation. In this context, alignment of corresponding sentences between a reference summary and its source documents has been leveraged to generate training data for some of the component tasks. Yet, this enabling alignment step has usually been applied heuristically on the sentence level on a limited number of subtasks. In this paper, we propose extending the summary-source alignment framework by (1) applying it at the more fine-grained proposition span level, (2) annotating alignment manually in a multi-document setup, and (3) revealing the great potential of summary-source alignments to yield several datasets for at least six different tasks. Specifically, for each of the tasks, we release a manually annotated test set that was derived automatically from the alignment annotation. We also release development and train sets in the same way, but from automatically derived alignments. Using the datasets, each task is demonstrated with baseline models and corresponding evaluation metrics to spur future research on this broad challenge.

==> derivedDatasets.tex <==

As described in Sections \ref{sec_intro} and \ref{sec_relatedWork}, prior works leveraged automatically-generated reference-source alignments at the sentence level to derive training datasets for several summarization subtasks. As shown in Section \ref{sec_sentExperiments}, deriving training data for sentence salience from our model's alignments yielded improved performance, relative to relying on prior alignment methods. Motivated by this result, 
in this section we show how our \infounit~alignments allow to systematically derive datasets for a full range of summarization-related tasks (see Table \ref{tab_tasks} and Fig. \ref{fig_derived_datasets}), represented at the finer proposition level, that open opportunities for future development of proposition-level models.
% As listed in Table \ref{tab_tasks} and illustrated in Figure \ref{fig_derived_datasets}, and detailed in the remainder of this section, our datasets span salience detection, information clustering and several generation steps, opening opportunities for future development of proposition-level models for these tasks.
As these tasks also stand on their own in additional NLP contexts, prior works dedicated targeted efforts to create individual datasets per task. Our dataset suite thus extends the inventory of datasets for these types of tasks, while attractively deriving all of them from a single ``pivot" information source, namely our \infounit~alignments.


To facilitate future research, we release dev, test and training datasets for each derived tasks (see statistics in Table \ref{tab_dataStat}). For each task, the dev and test datasets are derived from our corresponding crowdsourced alignment data (\sect \ref{sec_dataCollection}), providing exhaustive reliable annotations for tuning and testing task-specific models. 
To obtain training data, we follow the same methodology of prior work and Section \ref{sec_sentExperiments} and automatically generate alignments over large summarization datasets, using our supervised model. Specifically, we generate alignments for the multi-document summarization dataset MultiNews \citep{fabbri2019multinews} and for the single-document summarization dataset CNN/DailyMail \citep{Hermann2015TeachingMT} (note that all subtasks pertain also to the single-document setting, though at lower complexity). From these alignments, we derive a corresponding training dataset for each task. In addition, we derive smaller training datasets from our Pyramid-based alignments, used for training our \super$_{IU}$ (\sect \ref{sec_pyrData}), thus providing some more reliable yet modest-scale training data for each task.
















\subsection{Salience Detection}
\label{subsec_derived_salient}
Given an input set of documents to be summarized, the salience detection task identifies \textit{globally} important sentences or spans, with respect to the input document set. Salience models are often incorporated within summarization systems and related tasks (e.g. text highlighting \citep{Arumae2019TowardsAA}).
From our alignments, we derive a dataset of salient \infounit s, marking each \infounit~in a source document as salient if it is aligned with a summary \infounit~(see Figure \ref{fig_derived_datasets_sal} for illustration).
The number of salient \infounit s in each derived dataset is shown in Table \ref{tab_dataStat}. 




Notably, our dataset is the first to identify salience at the more focused proposition level, considering that a complete source sentence might include both salient and non-salient propositions. Further, our large scale training data is of relatively higher quality since it was derived from \super, which, as we showed, substantially outperforms ROUGE-based methods on which prior datasets were based. Finally, to the best of our knowledge, our dev and test salience datasets are the first to be based on exhaustive manual (alignment) annotation.




\subsection{Redundancy Clustering}
\label{subsec_derived_cluster}
In this task, the goal is to cluster together redundant paraphrastic pieces of information which roughly convey the same meaning. In summarization and related contexts, redundancy clustering may help generating texts that on the one hand are non-redundant and on the other hand fuse together partly-overlapping complementary pieces of information (as in \sect \ref{subsec_derived_generation}). Further, repetition of information across texts extracted by paraphrastic clustering typically indicates its importance, which was leveraged for salience detection via clustering \citep{Zhang2015ClusteringSW, Cai2010SimultaneousRA, Wan2008MultidocumentSU}. 

%Accordingly, a clustering task may be jointly modeled with salience task and may leverage their joint signal.


% In this task, the goal is to cluster together redundant paraphrastic pieces of information which (roughly) convey the same meaning. In summarization and related contexts, redundancy clustering helps generating texts that on the one hand are non-redundant and on the other hand fuse together related pieces of information (\sect \ref{subsec_derived_generation}). Paraphrastic clustering may be useful also in other contexts, such as text exploration and mining.


In our setting, we derive a proposition-level clustering dataset for all salient \infounit s in the source documents.
Given a document set and its reference summary, having a set of several source \infounit s aligned to the \textit{same} \infounit~in the reference implies that they are all paraphrastic (source \infounit s of the same-color, and same dash-type, in Figure \ref{fig_derived_datasets_alignment}). Accordingly, we form a gold cluster for each such set of \infounit s (illustrated in Figure \ref{fig_derived_datasets_cluster}). 
Table \ref{tab_dataStat} presents the total number of clusters and their average size for each of the clustering datasets.\footnote{Notice at this point that the alignment data supports also deriving a dataset for joint modeling of salience and clustering, by taking the input of the salience dataset (original documents) and the output of the clustering dataset (\infounit~clusters).}


To the best of our knowledge, our dataset is the first to provide paraphrastic clustering in an MDS context. Indeed, the prior works mentioned above, which employed clustering for summarization, did not evaluate explicitly their intermediate clustering phase, and applied only unsupervised clustering methods, due to the lack of suitable labeled clustering data.
In the broader context of paraphrasing, prior datasets typically present only paraphrase pairs \citep{Dolan2005AutomaticallyCA,Ganitkevitch2013PPDBTP}, while our dataset presents the broader challenge of clustering together all (salient) paraphrastic instances in a set of documents. 
Conversely, in the context of short text clustering, prior datasets typically cluster topically related instances, rather than paraphrastic ones \citep{phan2008classifyShortText, xu2017clusteringShortText}. 
Finally, we suggest that paraphrastic clustering is better captured at the proposition level, as in our dataset, rather than at the sentence level. This is since a pair of sentence might include some propositions that match in their content and some that don't, preventing the creation of coherent clusters.


% While we derived separate datasets for the salience and clustering tasks, 
% it is important to notice that our data also supports their joint modeling, where salience modeling may leverage the clustering signal. 
% This can be done by taking as input the full text of a given document set, as in the salience dataset, while considering the set of salient \infounit~clusters as output, as in the clustering dataset. Indeed, repetition of information across texts typically indicates its importance, which was leveraged for salience detection via  clustering \citep{Zhang2015ClusteringSW, Cai2010SimultaneousRA, Wan2008MultidocumentSU}.







\subsection{Generation}
\label{subsec_derived_generation}
% Text generation in MDS involves fusing salient information into a coherent summary. In this subsection, we derive datasets for two text generation subtasks, namely sentence planning and text realization, all capturing the fine-grained proposition level as described below. Here again, these datasets may be used individually, to develop models for the individual tasks, or may be merged together, to model these subtasks jointly. As an input representation, we use the \infounit~clusters generated in \sect \ref{subsec_derived_cluster}. Alternatively, one may use the unclustered raw salient \infounit s as input, without having to go through the clustering stage. In this alternative way, we can define a \textit{passage fusion} task to fit our data. We define \textit{passage fusion} as fusing a fairly large set of proposition spans, some of them redundant, into a coherent passage. While the common \textit{sentence} fusion task generates only a single sentence, most generation end-tasks, such as summarization and dialog, require generation of multiple sentences, which demands coherency at a larger scale.


Text generation in MDS involves fusing salient information into a coherent summary. In our context we consider a \textit{passage fusion} task, which requires fusing a fairly large set of proposition spans, some of them redundant, into a coherent passage. While the common \textit{sentence} fusion task generates only a single sentence, most generation end-tasks, such as summarization and dialog, require generation of multiple sentences, which demands coherency at a larger scale. In our case, the target of the fusion task would be outputting the reference summary, where the input is the set of all salient \infounit~s generated in \sect \ref{subsec_derived_salient}. Motivated by recent work \cite{Moryossef2019StepbyStepSP} in data-to-text generation, we propose to divide the fusion task to two steps: planning and realization. In their work, \citet{Moryossef2019StepbyStepSP} showed that an explicit text planning step, followed by a text realization step that generates the sentences text, improves overall generation quality compared to an end-to-end generation model. In our setup, we can easily derive dedicated training datasets for both planning and realization as explained below, which can be utilized to develop corresponding supervised models for these two subtasks.



\textbf{Sentence planning.} 
Sentence (or text) planning is a classical notion in the natural language generation literature (NLG) \cite{Reiter1997BuildingAN, Gatt2018SurveyOT}, approached in many variants. Here, we refer to the aspect of the planning task which determines how to partition the input units of information into an ordered set of sentences, to be subsequently generated.
% Within the NLG scope, some sentence planning datasets concern with structured data for dialog \citep{Walker2001SPoTAT, reed2018planning}, or text fragments for argument generation \citep{Hua2019ArgumentGW}, where most of them were created or labeled synthetically, sometimes followed by human judgment.
% Interestingly, recent work in data-to-text generation showed that an explicit text planning step, followed by a text realization step which generates the sentences text, improves overall generation quality compared to an end-to-end model \cite{Moryossef2019StepbyStepSP}.
Accordingly, we derive a novel sentence planning dataset, which corresponds to the MDS setting. For task input, we take all salient \infounit s generated in \sect \ref{subsec_derived_salient} for a given set of documents (topic). Then, as output, we partition the set of all \infounit s into ordered groups, each planned to generate an individual sentence. Based on the reference-source alignments, we group together all \infounit s that are aligned with reference \infounit s which appear in the same \textit{sentence} in the  summary. Further, we order these groups in the order of the corresponding sentences in the reference summary. In Figure \ref{fig_derived_datasets_gen} for example, the green and red document \infounit s are grouped together, aimed to be merged in the same sentence, because their aligned \infounit s appear in the same summary sentence, which is the first sentence in the summary.\footnote{Notice that sentence planning does not require in its output explicit redundancy clustering within each group of \infounit s corresponding to a planned sentence; we left the two cluster colors in the group corresponding to Sentence 1 only for easier tracking in the figure. Of course, redundancy clustering may be found useful to \textit{support} sentence planning.}
%Then, the yellow cluster gives rise to a next single planned sentence, because it aligns with a summary \infounit~that constitutes a sentence on its own (the second sentence of the summary), and so on.
In essence, this sentence planning gold data reconstructs the sentence planning decisions taken for the human reference summary.
Our dataset is unique in that it allows developing sentence planning models whose input consists of textual propositions. As complete sentences typically express several propositions, the proposition level provides a natural input unit for composing sentences in the sentence planning task.





\textbf{Text realization.} Given a sentence plan, the final subtask is text realization --- turning the plan representation into a coherent text passage \cite{Hua2019SentenceLevelCP,Moryossef2019StepbyStepSP}.
%In text-to-text generation, the realization phase may be viewed as addressing two main challenges. The first is generating each sentence by rephrasing and fusing one or more input text fragments \citep{barzilay2005fusion}, as designated in the sentence plan. The second challenge is ensuring global coherence of the full text, across all sentences, such as generating suitable referring expressions \citep{Zarrie2013CombiningRE}.
In our context, the input for a text realization instance is the sentence plan for the given document set (topic), consisting the ordered groups of salient \infounit s, where each group corresponds to a single sentence to be generated. The output is accordingly the reference summary for this topic.
In Figure \ref{fig_derived_datasets_gen}, the input consists of the three groups (red and green, yellow, blue), while the output is the three summary sentences (1, 2, 3). It is worth pointing out that sentence fusion may generally involve two different types of information fusion: fusing similar information by omitting redundancy \citep{thadani2013fusiondata}, versus combining different information into a coherent discourse structure \citep{geva2019discofuse}. These two different fusion types were often addressed separately in prior datasets, while our dataset poses the two challenges simultaneously. Table \ref{tab_dataStat} details the number of fused sentences in each text realization dataset (``\#sentences'').% and the average number of clusters per sentence.







% As mentioned in Section \ref{subsec:bg-ori}, there are two general types of fusion, one fuses similar information by omitting redundancy, and the second combines different information into a coherent discourse structure.
% While these fusion types were often addressed separately in prior datasets,  our dataset poses the two challenges simultaneously: \textit{Redundancy} fusion requires generating non-redundant text that expresses the redundant information in a proposition span cluster, while \textit{Discourse} fusion is required to combine multiple fused clusters into a single coherent sentence (sentence 1 in Figure \ref{fig_derived_datasets_gen}).

% It is worth pointing out that sentence fusion may generally involve two different types of information fusion. The first type is fusing inputs that primarily convey the same information, such as paraphrases. Here, the challenge is to generate a sentence that conflates redundancy while keeping complementary information \citet{thadani2013fusiondata}. The second type is combining several text fragments that convey different information into a single discourse-coherent sentence \citep{geva2019discofuse}. These two different fusion types were often addressed separately in prior datasets, while our dataset poses the two challenges simultaneously: redundancy fusion is required to generate a non-redundant text fragment verbalizing an \infounit~cluster, while discourse fusion is required to combine multiple fused clusters into a single sentence (sentence 1 in Figure \ref{fig_derived_datasets_gen}).




==> tables/table_tasks.tex <==
\begin{table*}[h!]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|l|l|l}
    
        \hline
         \textbf{Task} & \textbf{Input} & \textbf{Output} & \textbf{Derivable Annotations} \ran{Derived?}\\ \hline
         Highlighting & Doc set & Salient propositions & Annotated propositions only on source docs\\
         Coreference Clustering & Salient propositions & Clustered propositions & Linking of propositions with common aligned summ proposition\\
         Evidence Detection & Doc set \& summ proposition  & Mentions of the summ proposition& Linking of propositions with common aligned summ proposition\\

          Text Planning & Salient proposition clusters & Ordered Salient Proposition Groups & Propositional clusters that are linked to the same summary sentence\\
          Sentence Fusion & Salient proposition clusters & A fused sentence & Propositional clusters that are linked to the same summary sentence\\
          In-context Fusion & Doc set with marked propositions & Summary & Aligned source propositions are marked\\\hline
    
    \end{tabular}}
    
    \caption{Illustration of tasks whose annotations are potentially derivable from our dataset.\ran{instead of summ proposition maybe use S-prop and D-prop (summary proposition and document proposition and define in caption}}
    \label{tab_tasks}
\end{table*}
